Improving Compiler Bug Isolation by Leveraging Large Language Models

Compilers play a foundational role in building reliable software systems, and bugs within them can lead to catastrophic consequences. The compilation process typically involves hundreds of files, making traditional automated bug isolation techniques inapplicable due to scalability or effectiveness issues. Current mainstream compiler bug localization techniques have limitations in test program mutation and resource consumption. Inspired by the recent advances of pre-trained Large Language Models (LLMs), we propose an innovative approach named AutoCBI, which (1) uses LLMs to summarize compiler file functions and (2) employs specialized prompts to guide LLM in reordering suspicious file rankings. This approach leverages four types of information: the failing test program, source file function summaries, lists of suspicious files identified through analyzing test coverage, as well as compilation configurations with related output messages, resulting in a refined ranking of suspicious files. Our evaluation of AutoCBI against state-of-the-art approaches (DiWi, RecBi and FuseFL) on 120 real-world bugs from the widely-used GCC and LLVM compilers demonstrates its effectiveness. Specifically, AutoCBI isolates 66.67%/69.23%, 300%/340%, and 100%/57.14% more bugs than RecBi, DiWi, and FuseFL, respectively, in the Top-1 ranked results for GCC/LLVM. Additionally, the ablation study underscores the significance of each component in our approach.

==> background.tex <==
\section{BACKGROUND}
\label{sec:background}
%In this section, we first provide the background knowledge on test program mutation for compiler bug isolation and large language models (LLMs). 
\jiajun{This section can be removed if no space left.}
\subsection{Test Suite Enhancement for Compiler Bug Isolation}
Bug isolation is one of the most critical activities in software debugging. To address the issue of compiler bug isolation, Chen et al.\cite{chen2020survey} transformed this problem into the task of generating test programs. Given a failing test program that can trigger a compiler bug, existing methods first generate a passing test program that does not trigger the bug using different mutation strategies, thereby collecting the code coverage information of compiler source files. Based on Spectrum-Based Fault Localization (SBFL) theory\cite{sbfl1,sbfl2,sbfl3,sbfl4,sbfl5}, the compiler files touched during the compilation process by the failing test program are generally considered suspicious, while passing test programs help rule out unrelated files, with Ochiai\cite{ochiai} being a commonly used formula. Approaches like DiWi\cite{DiWi}, RecBi\cite{RecBi}, and LLM4CBI\cite{llm4cbi} all follow this idea.

Specifically, DiWi designed three types of local mutation operators, generating passing test programs by modifying three minimal elements of the failing test program: variables, constants, and operators. RecBi generates passing test programs through structured mutation operators to improve the efficiency of compiler bug isolation. LLM4CBI adopts a new method based on Large Language Models (LLMs) to achieve the same goal. This study aims to further leverage additional information, such as compiler file function descriptions, to assist LLM in more accurately identifying defective files in the compiler.
\subsection{Large Language Models (LLMs)}
In recent years, pre-trained Large Language Models (LLMs), such as ChatGPT\cite{chatgpt}, have seen widespread application across numerous fields and have demonstrated remarkable performance. These models not only excel in natural language processing tasks, such as machine translation, text summarization, question-answering systems, and dialogue generation, but also show great potential in more complex tasks like code generation and bug localization. LLMs, with their vast knowledge base and reasoning abilities, can execute a variety of downstream tasks based on simple task descriptions, without the need for fine-tuning or training on specific datasets. This capability is enabled through the use of prompts.

%Prompt engineering refers to designing the most effective task instructions for LLMs, enabling the model to understand and optimize its output\cite{wang2024prompt,marvin2023prompt}. By carefully crafting prompts, it is possible to significantly enhance the model's performance in specific tasks without requiring specialized training. Prompt engineering is not only applicable to traditional natural language processing tasks but has also proven effective in complex domains like code generation and bug localization. Previous studies have shown that prompt engineering can achieve state-of-the-art performance in various downstream tasks. For instance, in software debugging and bug fixing tasks, well-designed prompts can guide the model to generate more accurate code snippets or help pinpoint critical areas of a problem.

%This technological advancement is driven by the LLMs' ability to reason and understand complex contexts. Due to their ability to comprehend task details and quickly adapt to new problem scenarios, LLMs are increasingly being applied in software engineering, especially in automated tasks. This includes fields such as automatic code generation, code repair, debugging, and code review generation. These applications not only reduce the need for human intervention but also accelerate the development cycle and improve overall efficiency.

Inspired by the immense potential of LLMs, recent studies have increasingly highlighted the broad application potential of LLMs in solving software engineering problems\cite{jin2023inferfix,zhang2024autocoderover}. For example, LLMs have been applied to tasks such as code snippet generation\cite{jin2023inferfix}, bug localization\cite{do2023using}, and code optimization\cite{zhang2024autocoderover}. In these tasks, LLMs can generate high-quality code or provide reasonable solutions to complex problems based on natural language descriptions, greatly reducing the time and effort required by developers during the debugging and fixing stages.

In bug localization, LLMs have demonstrated great potential\cite{kang2024quantitative}. Traditional bug localization methods often rely on extensive testing and complex analysis tools, while LLMs can quickly generate candidate solutions based on natural language prompts or code descriptions, assisting developers in identifying the source of the problem. For example, LLMs can generate potential error areas and suggest fixes based on given error logs, code context, and test results. This capability not only improves software development efficiency but also lays the foundation for more intelligent debugging tools.

LLMs can be broadly divided into two categories: fill-in models and general models. Fill-in models (such as CodeGen\cite{nijkamp2022codegen}, Incoder\cite{fried2022incoder}, and PolyCoder\cite{xu2022systematic}) are primarily used to insert the most natural code snippets based on bidirectional context, making them suitable for scenarios where new content needs to be inserted into an existing code context. These models are well-suited for handling code completion tasks, filling in logical gaps between known code blocks. General models (such as LLaMA\cite{touvron2023llama}, Alpaca\cite{maeng2017alpaca}, and ChatGPT\cite{chatgpt}) focus on generating complete code snippets based on natural language descriptions and left-side context.

In this study, we selected general models for compiler bug localization. These models, with their ability to engage in prompt-driven conversations, can generate task-specific responses based on given prompts. Compared to fill-in models, general models offer greater flexibility, enabling them to generate more complex code or problem analysis based on natural language descriptions. By incorporating additional information into the model, such as compiler file function summaries and coverage differences between failing and passing test cases, we can further enhance the performance of LLMs in bug localization. The introduction of multi-source information provides the model with more background and context, allowing it to understand the problem more precisely and perform more efficient bug localization within compiler files.

==> tab-component.tex <==
\begin{table*}[tbp]
\caption{Performance of \tool{} when disabling each component in it.}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc|cc|cc} 

\toprule
\textbf{Subject}&\textbf{Approach}&\textbf{Top-1}&\textbf{\textuparrow Top-1}&     \textbf{Top-5}&\textbf{\textuparrow Top-5}&\textbf{Top-10}&\textbf{\textuparrow Top-10}&\textbf{Top-20}&\textbf{\textuparrow Top-20}&\textbf{MFR}&\textbf{\textuparrow MFR}&\textbf{MAR}&\textbf{\textuparrow MAR}\\ 
\midrule
\rowcolor{gray!40} \cellcolor{white}
\multirow{9}*{GCC}& \tool{}
& \textbf{20} &/&     33 &/&\textbf{39} &/&\textbf{45} &/&\textbf{7.71} &/&\textbf{9.22} &/\\ 

& \variant{-summary}& 10 &-50.00\%&      25 &-24.24\%&34 &-12.82\%&39 &-13.33\%&12.60  &-63.42\%&16.62
 &-80.26\%\\ 
& \variant{-compile}& 9 &-55.00\%& 26 &-21.21\%&33 &-15.38\%&40 &-11.11\%&13.41  &-73.93\%&
 17.2
 &-86.55\%\\
 & \variant{-execov}& 11 &-45.00\%& 21 &-36.36\%& 34 &-12.82\%& 40 &-11.11\%& 11.81  &-53.18\%&15.64
 &-69.63\%\\
  & \variant{-testcov}& 14 &-30.00\%&      25 &-24.24\%&34 &-12.82\%&42 &-6.67\%&10.06  &-30.48\%&14.28
 &-54.88\%\\ 
& \variant{-llm}& 14&-30.00\%& 23&-30.30\%& 29&-25.64\%& 40 &-11.11\%& 12.08&-56.68\%&16.06&-74.19\%\\
& \variant{-failtest}& 9 &-55.00\%&      21 &-36.36\%&33 &-15.38\%&39 &-13.33\%&12.56  &-62.91\%&16.60
 &-80.04\%\\ 

  & \variant{+deepseekv3}& 16 &-20.00\%&     34 &3.03\%&36 &-7.69\%&42 &-6.67\%&10.76  &-39.56\%&12.13
 &-31.56\%\\ 
  & \variant{+deepseekr1}& 16 &-20.00\%&     \textbf{35} &\textbf{6.06\%}&\textbf{39}&\textbf{0.00\%}&42 &-6.67\%&9.96  &-29.18\%&11.5
 &-24.73\%\\ 
% & \variant{+gpt4turbo}& 18 &-10.00\%& 29 &-12.12\%& 38 &-2.56\%& 44 &-2.22\%& 9.46  &-22.70\%&13.62 &-47.72\%\\
\midrule
\rowcolor{gray!40} \cellcolor{white}
 \multirow{9}*{LLVM}& \tool{}
& \textbf{22} &/& 30 &/& \textbf{39} &/& 50 &/& \textbf{8.70} &/&\textbf{10.25} 
 &/\\
 & 
\variant{-summary}
& 11 &-50.00\%& 21 &-30.00\%& 30 &-23.08\%& 45 &-10.00\%& 12.57  &-44.48\%&12.65 
 &-23.41\%\\
 & \variant{-compile}
& 14 &-36.36\%& 24 &-20.00\%& 35 &-10.26\%& 46 &-8.00\%& 10.82  &-24.37\%&11.53 
 &-12.49\%\\
 & \variant{-execov}
& 14 &-36.36\%& 24 &-20.00\%& 33 &-15.38\%& 46 &-8.00\%& 12.60  &-44.83\%&12.79 
 &-24.78\%\\
  & \variant{-testcov}& 15 &-31.82\%&      26 &-13.33\%&36 &-7.69\%&\textbf{52} &\textbf{4.00\%}&9.35  &-7.47\%&10.74
 &-4.78\%\\ 
& \variant{-llm}& 16 &-27.27\%& 25 &-16.67\%& 36 &-7.69\%& 50 &0.00\%& 9.73&-11.84\%&11.12&-8.47\%\\
% & \variant{+gpt4turbo}& 21 &-4.55\%& 29 &-3.33\%& \textbf{40} &\textbf{2.56\%}& \textbf{51} &\textbf{2.00\%}& 9.05  &-4.02\%&\textbf{9.24} &\textbf{9.85\%}\\
& \variant{-failtest}& 10&-54.55\%&      21 &-30.00\%&33 &-15.38\%&45 &-10.00\%&12.80  &-47.13\%&13.05
 &-27.32\%\\ 

   & \variant{+deepseekv3}& 16 &-27.27\%&     28 &-6.67\%&36 &-7.69\%&48 &-4.00\%&10.08  &-15.86\%&11.62
 &-13.37\%\\ 
  & \variant{+deepseekr1}& 16 &-27.27\%&    \textbf{31} &\textbf{3.33\%}&\textbf{39} &\textbf{0.00\%}&48 &-4.00\%&9.67  &-11.15\%&11.05
 &-7.80\%\\ 
\bottomrule
\multicolumn{14}{l}{*Columns "\textuparrow" present the improvement rates of experiment variants over \tool{} in terms of various measurements.}\\
\end{tabular}
}
\label{tab2}
\end{center}
\end{table*}

==> tab-formula.tex <==
\begin{table*}[tbp]
\begin{center}
\caption{Performance of \tool{} when adopting different SBFL formulas.}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc|cc|cc} 

\toprule
\textbf{Subject}&\textbf{Approach}&\textbf{Top-1}&\textbf{\textuparrow Top-1}&     \textbf{Top-5}&\textbf{\textuparrow Top-5}&\textbf{Top-10}&\textbf{\textuparrow Top-10}&\textbf{Top-20}&\textbf{\textuparrow Top-20}&\textbf{MFR}&\textbf{\textuparrow MFR}&\textbf{MAR}&\textbf{\textuparrow MAR}\\ 
\midrule
\rowcolor{gray!40} \cellcolor{white}
\multirow{9}*{GCC}& \tool{}
& \textbf{20} &/&     \textbf{33} &/&\textbf{39} &/&\textbf{45} &/&\textbf{7.71} &/&\textbf{9.22} &/\\ 

& \variant{+Ochiai[exec]}& 18 &-10.00\%&      30 &-9.09\%&36 &-7.69\%&44 &-2.22\%&10.21  &-32.43\%&14.28
 &-54.88\%\\ 

 & \variant{+Barinel[exec]} & 18 &-10.00\%& 28 &-15.15\%&36 &-7.69\%&45 &0.00\%&9.75  &-26.46\%&
 11.76
 &-27.55\%\\
 & \variant{+DStar2[exec]}& 17 &-15.00\%& 27 &-18.18\%& 36 &-7.69\%& 43 &-4.44\%& 10.60  &-37.48\%&12.54
 &-36.01\%\\
 & \variant{+Tarantula[exec]}& 17 &-15.00\%& 28 &-15.15\%& 36 &-7.69\%& 42 &-6.67\%& 10.58  &-37.22\%&14.76
 &-60.09\%\\
\cline{2-14}
% % \multirow{5}*{GCC}& AutoCBI
% & \textbf{20} &/&     \textbf{33} &/&39&/&45&/&\textbf{7.71} &/&\textbf{9.22} &/\\ 
& \variant{+Wong2[test]}
& 19
&-5.00\%&      32
&-3.03\%&38
&-2.56\%&\textbf{46}&\textbf{2.22\%}&8.81
&-14.27\%&9.28
&-0.56\%\\ 
 & \variant{+Barinel[test]}& 19
&-5.00\%& 32
&-3.03\%&38
&-2.56\%&45
&0.00\%&8.22
&-6.61\%&
 9.36
&-1.52\%\\
 & \variant{+DStar2[test]}& \textbf{20}&\textbf{0.00\%}& 32
&-3.03\%& 41
&5.13\%& 45
&0.00\%& 8.33
&-8.04\%&9.72
&-5.42\%\\
 & \variant{+Tarantula[test]}& 18
&-10.00\%& \textbf{33}&\textbf{0.00\%}& \textbf{42}&\textbf{7.69\%}& 45
&0.00\%& 8.08
&-4.80\%&9.64
&-4.56\%\\
 
\midrule
\rowcolor{gray!40} \cellcolor{white}
 \multirow{9}*{LLVM}& \tool{}
& \textbf{22} &/& \textbf{30} &/& 39 &/& 50 &/& 8.70 &/&10.25 
 &/\\
 & 
\variant{+Ochiai[exec]}
& 15 &-31.82\%& 27 &-10.00\%& \textbf{40} &\textbf{2.56\%}& 50 &0.00\%& 9.04  &-3.91\%&9.88 
 &3.61\%\\
 & \variant{+Barinel[exec]} 
& 18 &-18.18\%& \textbf{30}&\textbf{0.00\%}& \textbf{40} &\textbf{2.56\%}& \textbf{54} &\textbf{8.00\%}& \textbf{8.24} &\textbf{5.29\%}&\textbf{8.29} &\textbf{19.12\%}\\
 & \variant{+DStar2[exec]}
& 19 &-13.64\%& 29 &-3.33\%& 39 &0.00\%& 52 &4.00\%& 9.15  &-5.17\%&9.16 
 &10.63\%\\
 & \variant{+Tarantula[exec]}& 18 &-18.18\%& 27 &-10.00\%& 38 &-2.56\%& 49 &-2.00\%& 9.63  &-10.69\%&11.17 
 &-8.98\%\\
\cline{2-14}
& 
\variant{+Wong2[test]}
& 21
&-4.55\%& \textbf{30}&\textbf{0.00\%}& 38
&-2.56\%& 50
&0.00\%& 8.72 
&-0.23\%&10.28 
&-0.29\%\\
 & \variant{+Barinel[test]}& \textbf{22}&\textbf{0.00\%}& \textbf{30}&\textbf{0.00\%}& \textbf{40}&\textbf{2.56\%}& 50
&0.00\%& \textbf{8.46}&\textbf{2.76\%}&\textbf{10.02}&\textbf{2.24\%}\\
 & \variant{+DStar2[test]}
& 21
&-4.55\%& \textbf{30}&\textbf{0.00\%}& 38
&-2.56\%& \textbf{51}&\textbf{2.00\%}& 8.74 
&-0.46\%&10.30 
&-0.49\%\\
 & \variant{+Tarantula[test]}& 21
&-4.55\%& 29
&-3.33\%& 39
&0.00\%& 50
&0.00\%& 8.63 
&0.80\%&10.20 
&0.49\%\\
 
\bottomrule
\multicolumn{14}{l}{*Columns "\textuparrow" present the improvement rates of experiment variants over \tool{} in terms of various measurements.}\\
\end{tabular}
}
\label{tab3}
\end{center}
\end{table*}
